Xkernel: Principled Performance Tunability of Operating System Kernels

The Linux kernel is permeated with constant values that are critical to system performance. Many of these constants, referred to as perf-consts, are magic numbers with brittle assumptions on hardware and workloads. Unfortunately, there is no capability of in-situ tuning of perf-const values on deployed kernels. This paper rethinks OS performance tunability. We present Xkernel, a system that offers a safe, efficient, and programmable interface for in-situ tuning of any perf-consts directly on a running kernel. Xkernel transforms any perf-const into a tunable knob on demand using a novel approach called Scoped Indirect Execution (SIE). SIE captures precise binary boundaries where a perf-const enters system state and redirects control to synthesized instructions that update the state as if new values were used. Xkernel goes beyond version atomicity when updating perf-consts to guarantee side-effect safety, a property notably absent in existing kernel update mechanisms. Case studies on various OS subsystems demonstrate significant performance benefits of tuning perf-consts which is made possible by Xkernel.

==> 4_0_design_overviewfirst.tex <==

\subsection{Overview}

% This is the system

\sysname{} is a system that realizes the principled performance tunability
  for OS kernels defined in \S\ref{sec:tunability}.
We implemented \sysname{} on Linux.
\sysname{} offers a safe, efficient, and programmable interface 
  for {\it in-situ} tuning of any \perfconsts directly on a deployed Linux kernel.
%  without (re)compiling or rebooting the kernel.
% \sysname essentially transforms a \perfconst into a tunable knob on demand,
%  which can be updated safely at runtime.
% \sysname{} is efficiently for online performance tuning at the microsecond scale.
% Its expressive and programmable interface can support fine-grained tuning policies
%  and can be used by tuning programs or agents.
Figure~\ref{fig:xkernel-arch} gives an overview of \sysname
  and its user-facing workflow.
\sysname{} performs {\it offline} static analysis on kernel code to understand 
  the scope of each \perfconst{} based on how each \perfconst{} is used in kernel instructions and 
  affects kernel runtime states; the scope information is 
  encoded in a data structure termed critical span (CS).
It then synthesized code to update the kernel states related to the \perfconst
  using a novel technique termed {\it Scoped Indirect Execution}.
\sysname{} also captures the transition points in the kernel code 
  that ensures safe transition from the original \perfconst{} value to a new value;
  the information is encoded in a data structure termed safe span (SS).
\sysname{} maintains the CSes and SSes of each \perfconst{} in a global Scope Table.
% Each entry maps the constant's ID (i.e., source location) 
%  to its symbolic state expression, critical spans, and safe spans
% (labeled as expression, CS, and SS in Figure~\ref{fig:xkernel-arch}). 
Note that the offline analysis is one-time effort.
The scope table only needs to be updated when the deployed kernel is updated.
% \sysname can build this table ahead of time for any set of constants; this cost is paid
% once per constant.

To tune a \perfconst{} at runtime, the user (or agent) specifies the \perfconst{}
  in the source code (defined by the source file, line number, and token index),
  and implements tuning policy code, called X-tune, in BPF.
X-tune can be loaded at any point during the OS execution. A lightweight
runtime (\xkruntime) handles attachment and safe transitions.

% invokes \xkgen\ with the
% constant's ID. \xkgen\ generates a skeleton program exposing a programmable
% interface (e.g., \smalltt{xk\_set()}); the user then edits the skeleton to
% implement their tuning policy.

% When a \xkprog\ is loaded, \xkruntime\ consults the \xktable\ to determine the
% relevant binary spans, synthesizes the required indirections, and feeds both the
% user policy and the synthesized code into the eBPF JIT to produce bytecode.
% These details remain internal and invisible to the user. \xkruntime\ then
% initiates transitioning, with side-effect safety guaranteed by the safe spans.

% Once transitioning completes, any execution that reaches an attached indirection
% point is redirected to the generated instructions. The externally visible
% behavior is ensured to reflects the updated value once execution has passed the
% critical span.


\input{fig-tex/fig-xkernel-arch.tex}

\minisec{Scoped Indirect Execution (SIE)}
\label{sec:sie}
% This is the idea/approach
% want people to understand what we do from the high level
SIE is the key approach of \sysname{} that realizes safe and efficient
  \perfconst{} tuning.
% the core insight: what's unique about constant
The insight is that \perfconsts exhibit intrinsic
  instruction-level semantics.
% that shed light on in-situ tuning without recompilation or reboot. 
For a \perfconst, the point where its value
enters the architectural state forms a {\em well-scoped boundary}. 
% naturally separating the tuning mechanism from the programmable policy.
% property of the scope (constant's effects)
Each boundary---a {\em critical span}---has 
  three properties: 
  (1) it can be localized by static analysis,
% the constant appears as a literal (possibly transformed) determined entirely by the compiler. 
% Second, 
  (2) it corresponds to a {\em symbolic state expression} that
  captures the relation between the state and the \perfconst, 
% despite compiler optimizations that may alter instruction forms. Third, 
(3) the boundary is {\em small}, involving only a few instructions, which keeps correctness
reasoning narrow and makes safe runtime adaptation tractable.

% how the SIE works
% this is the core of SIE, others are used to make it work
SIE identifies the critical span based on the symbolic state expression and
safely redirects execution, at runtime, to a short JIT-compiled instruction
sequence. These instructions execute adjacent to the original code and, when
combined with it, produce the same effects as if the \perfconst{} was changed
directly. The original binary remains intact; all modification occurs
indirectly, within scoped regions.

\if 0
% the indirection -- source code
The JIT input combines a user policy with synthesized source codes tied to
its invocation site; we call these {\em SIE indirections}. They are synthesized
based on the recovered symbolic state expression, which provides correctness
guarantees for runtime updates without recompilation.
\fi

% second scope: it is analyzed from the expression
SIE also ensures side-effect safety by defining a second binary scope, the {\em safe
span}, within which the effects of the constant (i.e., the expression) are propagated,
consumed, and fully contained. Transitioning occur only when execution is outside this
span, converting a temporal coordination problem into a spatial one that can be
analyzed statically. % based on the precisely recovered expression. 

==> Makefile <==
MAIN      = main
SRCS      = *.tex 
TARG      = $(MAIN).pdf
ARGS      = -shell-escape


all: $(TARG)

pdf: $(SRCS) $(MAIN).bbl
	pdflatex $(ARGS) $(MAIN)
	source ./SourceMe ; \
	pdflatex $(ARGS) $(MAIN)
	#cp main.pdf ~/Dropbox/Documents/

$(TARG): $(SRCS) $(MAIN).bbl
	pdflatex $(ARGS) $(MAIN)
	pdflatex $(ARGS) $(MAIN)
	touch $(TARG)
	#cp main.pdf ~/Dropbox/Documents/

bib: $(MAIN).bbl bib.tex

$(MAIN).bbl: $(MAIN).aux
	bibtex -min-crossrefs=100 $(MAIN)
	# The below line is commented because usenix started checking
	# formatting for references also -- running redo-bib would 
	# squish the references without space to which the format 
	# checker would complain! 
	#./redo-bib.csh $(MAIN)

$(MAIN).aux: $(MAIN).tex
	pdflatex $(ARGS) $(MAIN)

clean:
	rm -f $(TARG) *.aux *~ $(MAIN).log $(MAIN).bbl $(MAIN).blg $(MAIN).out $(MAIN).dep

.SECONDARY: $(DVI)


==> fig-tex/fig-cases-results.tex <==

\begin{figure*}[t!]
    \centering
    % First figure (25%)
    \begin{minipage}[b]{0.26\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth]{figs/cs1-crop.pdf}
        \caption{Cost-benefit tradeoff that can be tuned 
            by changing values of \MaxSoftirqRestartTt.}
        \label{fig:cases:softirq}
    \end{minipage}
    \hfill
    % Second figure (29%)
    % \begin{minipage}[b]{0.28\textwidth}
    \begin{minipage}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth]{figs/cs2-crop.pdf}
        \caption{Tuning \ShrinkBatchTt{} can significantly 
            reduce write latency of the workload.}
        \label{fig:cases:shrinker}
    \end{minipage}
    \hfill
    % Third figure (45%)
    % \begin{minipage}[b]{0.45\textwidth}
    \begin{minipage}[b]{0.44\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/cs3-crop.pdf}
        \caption{Tuning \NrMaxBatchedMigrationTt{} to reduce tail latency, 
            which requires understanding TLB shootdown behavior.}
% \todo{@tianyin -- CPU TLB shootdown: invalidate TLB entries on other CPU cores; Remote IPI Send: request other CPU cores to invalidate TLB entries.}}
        \label{fig:cases:numa}
    \end{minipage}

    % \caption{\textbf{Performance Improvement of Cases in Table~\ref{tab:case-study}}. (c) CPU TLB shootdown: invalidate TLB entries on other CPU cores; Remote IPI Send: request other CPU cores to invalidate TLB entries.}
    \label{fig:cases}
\end{figure*}

==> fig-tex/fig-eval-const-categories.tex <==
\begin{figure}[t!] 
  \centering
  \includegraphics[width=\columnwidth]{figs/dataset_distribution-crop.pdf}
  \caption{Characteristics of the evaluated \perfconsts
  The categories are specified in Table~\ref{tab:perf-const-categories}.}
  \label{fig:dataset-src}
\end{figure}

==> table-ir.tex <==
% env->loop_break += SCHED_NR_MIGRATE_BREAK;

% (+0xe86)ffffffff8f7f4406:       83 c1 20                add    $0x20,%ecx
% (+0xe89)ffffffff8f7f4409:       83 4d a8 02             orl    $0x2,-0x58(%rbp)
% (+0xe8d)ffffffff8f7f440d:       4c 8b bd 50 ff ff ff    mov    -0xb0(%rbp),%r15
% (+0xe94)ffffffff8f7f4414:       89 4d b0                mov    %ecx,-0x50(%rbp)

\begin{table*}[t!]
\centering
\small
\caption{Diff instructions and Critical Spans for different cases.}
\label{tab:ir}
\begin{tabular}{p{0.3\linewidth} p{0.25\linewidth} p{0.25\linewidth}}
\toprule 
\textbf{C Example} & \textbf{Critical Span} & \textbf{$V$ in Symbolic Execution} \\
\midrule 
\texttt{q->nr\_requests = \textbf{128;}} & \texttt{\textbf{\textcolor{blue}{movq \$0x80, 0x170(\%rbx);}}} 
& \textbf{\texttt{0x80}}
\\
\midrule
\texttt{if (gro\_list->count >= \textbf{8})} & \texttt{mov    0x50(\%rdx),\%eax} \newline \texttt{\textbf{\textcolor{blue}{cmp \$0x7, \%eax;}}} \newline \texttt{jg     0xffffffff9980496e} \newline \texttt{add    \$0x1,\%eax} & \textbf{\texttt{0x7}}
\\
\midrule
\texttt{q->nr\_requests = 2 * min\_t(unsigned} \newline \texttt{int, q->tag\_set->queue\_depth, \textbf{128})} & \texttt{mov 0x40(\%rdi), \%eax;} \newline \texttt{\textbf{\textcolor{blue}{mov \$0x80, \%edx;}}} \newline \texttt{cmp \%edx, \%eax;} \newline \texttt{cmova \%edx, \%eax;} \newline \texttt{add \%eax, \%eax;} \newline \texttt{mov \%rax, 0x170(\%rbx);} & \textbf{\texttt{0x80}}
\\
\midrule
\texttt{env->loop\_break += \textbf{32};} & \texttt{\textbf{\textcolor{blue}{add \$0x20,\%ecx;}}} \newline \texttt{{mov \%ecx,-0x50(\%rbp);}} 
& \textbf{\texttt{0x20}}
\\
\midrule
\texttt{static inline unsigned short} \newline \texttt{\quad blk\_plug\_max\_rq\_count(} \newline \texttt{\quad struct blk\_plug *plug)\{} \newline \texttt{\quad if (plug->multiple\_queues)} \newline \texttt{\quad \quad return \textbf{32} * 2;} \newline \texttt{\quad return \textbf{32};} \newline \texttt{\}}\newline \texttt{if (plug->rq\_count >=} \newline \texttt{\quad blk\_plug\_max\_rq\_count(plug))} & \texttt{cmp \$0x1, \%r13b;} \newline \texttt{\textbf{\textcolor{blue}{sbb \%eax, \%eax;}}} \newline \texttt{{\textbf{\textcolor{blue}{and \$0xffffffe0, \%eax;}}}} \newline \texttt{\textbf{\textcolor{blue}{add \$0x40, \%eax;}}} \newline \texttt{cmp \%ax, \%r14w} \newline \texttt{jae    0xffffffff8fe8f8a5}
& \texttt{\%eax = \textbf{0x20}}
\\
\midrule
\texttt{\#define fits\_capacity(cap, max) \newline ((cap) * \textbf{1280}} \texttt{\quad < (max) * 1024)} & \texttt{\textbf{\textcolor{blue}{lea (\%r14,\%r14,4),\%rcx;}}} \newline \texttt{\textbf{\textcolor{blue}{shl \$0x8, \%rcx;}}} \newline \texttt{mov 0xb90(\%rax,\%rdi,1),\%rax;} \newline \texttt{shl \$0xa, \%rax;} \newline \texttt{cmp \%rax, \%rcx;} \newline \texttt{setb \%cl} 
& \texttt{\%rcx = \textbf{1280} * \%r14}
\\
\bottomrule
\end{tabular}
\end{table*}

% \begin{table*}[t]
% \centering
% \small
% \caption{Instruction Sequence Types for \const Tuning.}
% \label{tab:ir}
% \begin{tabular}{l l p{0.3\linewidth} p{0.3\linewidth}}
% \toprule  
% \textbf{Sequence Type} & \textbf{Frequency} & \textbf{C Example} & \textbf{Instruction sequence} \\
% \midrule 
% (1) DTI-Only          & Common             & \texttt{q->nr\_requests=\textbf{BLKDEV\_DEFAULT\_RQ};} & \texttt{\textbf{\textcolor{blue}{movq \$0x80, 0x170(\%rbx);}}} \\
% \midrule
% (2) CI-Only           & Common             & \texttt{if (unlikely(gro\_list->count >=} \newline \texttt{\quad \textbf{MAX\_GRO\_SKBS}))} & \texttt{mov    0x50(\%rdx),\%eax} \newline \texttt{\textbf{\textcolor{blue}{cmp \$0x7, \%eax;}}} \newline \texttt{jg     0xffffffff9980496e} \newline \texttt{add    \$0x1,\%eax} \\
% \midrule
% (3) DTI + CI   & Common             & \texttt{q->nr\_requests = 2 * min\_t(unsigned} \newline \texttt{int, q->tag\_set->queue\_depth,} \newline \texttt{\quad \textbf{BLKDEV\_DEFAULT\_RQ});} & \texttt{mov 0x40(\%rdi), \%eax;} \newline \texttt{\textbf{\textcolor{blue}{mov \$0x80, \%edx;}}} \newline \texttt{cmp \%edx, \%eax;} \newline \texttt{cmova \%edx, \%eax;} \newline \texttt{add \%eax, \%eax;} \newline \texttt{mov \%rax, 0x170(\%rbx);} \\
% \midrule
% (4) ALI + DTI          & Common             & \texttt{env->loop\_break +=} \newline \texttt{\textbf{SCHED\_NR\_MIGRATE\_BREAK};} & \texttt{\textbf{\textcolor{blue}{add \$0x20,\%ecx;}}} \newline \texttt{{mov \%ecx,-0x50(\%rbp);}} \\
% \midrule
% (5) ALI + CI       & Rare          & \texttt{static inline unsigned short} \newline \texttt{\quad blk\_plug\_max\_rq\_count(} \newline \texttt{\quad struct blk\_plug *plug)\{} \newline \texttt{\quad if (plug->multiple\_queues)} \newline \texttt{\quad \quad return \textbf{BLK\_MAX\_REQUEST\_COUNT} * 2;} \newline \texttt{\quad return \textbf{BLK\_MAX\_REQUEST\_COUNT};} \newline \texttt{\}}\newline \texttt{if (plug->rq\_count >=} \newline \texttt{\quad blk\_plug\_max\_rq\_count(plug))} & \texttt{cmp \$0x1, \%r13b;} \newline \texttt{sbb \%eax, \%eax;} \newline \texttt{{\textbf{\textcolor{blue}{and \$0xffffffe0, \%eax;}}}} \newline \texttt{\textbf{\textcolor{blue}{add \$0x40, \%eax;}}} \newline \texttt{cmp \%ax, \%r14w} \newline \texttt{jae    0xffffffff8fe8f8a5}\\
% \midrule
% % (6) DTI + ALI + CI & Rare             & \texttt{\#define fits\_capacity(cap, max) \newline ((cap) * 1280} \texttt{\quad < (max) * \textbf{1024})} & \texttt{lea (\%r14, \%r14, 4), \%rcx;} \newline \texttt{shl \$0x8, \%rcx;} \newline \texttt{mov 0xb90(\%rax, \%rdi, 1), \%rax;} \newline \texttt{\textbf{\textcolor{blue}{shl \$0xa, \%rax;}}} \newline \texttt{cmp \%rax, \%rcx;} \newline \texttt{setb \%cl} \\
% (6) DTI + ALI + CI & Rare             & \texttt{\#define fits\_capacity(cap, max) \newline ((cap) * \textbf{1280}} \texttt{\quad < (max) * 1024)} & \texttt{\textbf{\textcolor{blue}{lea (\%r14, \%r14, 4), \%rcx;}}} \newline \texttt{\textbf{\textcolor{blue}{shl \$0x8, \%rcx;}}} \newline \texttt{mov 0xb90(\%rax, \%rdi, 1), \%rax;} \newline \texttt{shl \$0xa, \%rax;} \newline \texttt{cmp \%rax, \%rcx;} \newline \texttt{setb \%cl} \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> tbl-tex/tbl-cases.tex <==
\begin{table*} %[h]
% \small
\footnotesize
\centering
\setlength{\tabcolsep}{4pt}
\caption{Summary of case studies that demonstrate \sysname's features and capabilities.}
\begin{tabular}{llcl}
\toprule
\textbf{Perf-const} & \textbf{Subsystem} & \textbf{Default} & {\bf Performance Tuning Regime} \\
\midrule
\BlkMaxReqCntTt\         & Storage (Block layer)       & 32   & Adapting to hardware devices and workload patterns (see \S\ref{sec:def}) \\
\MaxSoftirqRestartTt\    & CPU (Interrupt)             & 10   & Tradeoffs between tail latency and CPU utilization \\
\ShrinkBatchTt\          & Memory (Reclamation)        & 128  & Controlling kernel internal behavior (e.g., maintenance) \\
\NrMaxBatchedMigrationTt & Memory (Page migration)     &  512 & Tuning with kernel and hardware observability \\
\HystartDelayTt[\smalltt{MAX}, \smalltt{MIN}, factor] & Network (TCP CUBIC)  & [16, 4, 3] $\ $ & Collective tuning of interdependent \perfconsts \\
\bottomrule
\end{tabular}
\label{tab:case-study}
\end{table*}
